Towards Models that Can See and Read

Visual Question Answering (VQA) and Image Captioning (CAP), which are among the most popular vision-language tasks, have analogous scene-text versions that require reasoning from the text in the image. Despite their obvious resemblance, the two are treated independently and, as we show, yield task-specific methods that can either see or read, but not both. In this work, we conduct an in-depth analysis of this phenomenon and propose UniTNT, a Unified Text-Non-Text approach, which grants existing multimodal architectures scene-text understanding capabilities. Specifically, we treat scene-text information as an additional modality, fusing it with any pretrained encoder-decoder-based architecture via designated modules. Thorough experiments reveal that UniTNT leads to the first single model that successfully handles both task types. Moreover, we show that scene-text understanding capabilities can boost vision-language models' performance on general VQA and CAP by up to 2.69% and 0.6 CIDEr, respectively.

==> Rebuttal_Tables/blip_large.tex <==
\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{l | c c c c c c c}
        \toprule	 	
        \multirow{2}{*}{\textbf{Method}} &   \multicolumn{2}{c}{\textbf{VQA}} & \multicolumn{2}{c}{\textbf{TextVQA}} & \textbf{ST-VQA} & \textbf{COCO} & \textbf{TextCaps} \\
        & test-dev & test-std & val & test & test-ANLS & CiDER & CiDER \\
        \midrule
        $\text{BLIP}_{\text{large}}$  & ? & ? & ? & ? & ? & 136.7 & 60.04\\
        + Comb.  & 77.3 & ? & 32.37 & ? & ? & 136.2 & 92.09 \\
        + \AlgoName  & ? & ? & ? & ? & ? & \textbf{136.8} & \textbf{105.71} \\
	    \bottomrule
	\end{tabular}
        }
        \vspace{-0.2cm}
        \tiny
	\caption{
            The effect of UniTnT on BLIP-Large, in color the gap from Comb.}
	\label{table:blip_large}
\vspace{-0.3cm}
\end{table}

==> Rebuttal_Tables/caps_ablation.tex <==
\begin{table}
% \vspace{-0.5cm}
% \normalsize
\begin{center}

\small
\bgroup
\def\arraystretch{1.1}
    \resizebox{1\linewidth}{!}{%
        \begin{tabular}{l | cccccc}
        \toprule
        Component & \textbf{Comb.} &+\textbf{OCR-Sys} & +\textbf{OCR-Enc} & +\textbf{Fuse} & +${\mathcal{L}_{OCR-LM}}$ & +\textbf{2-D}\\ 
        \midrule
        % ALBEF \cite{albef} & 12.31 & 5.77 & \color{Red}{6.54} \\
        % BLIP \cite{li2022blip} & 21.12 & 15.19 & \color{Red}{5.93}\\
        % OFA \cite{ofa} & 17.07 & 13.27 & \color{Red}{3.80} \\
        COCO     & 133.4 & 133.5 & 133.5 & 133.5 & 133.8 & 134.0 \\
        TextCaps & 101.4 & 109.73 & 110.41 & 118.32 & 118.9 & 119.13\\
        % \midrule
        % \AlgoNameALBEF & 44.07 & 33.77 & \textbf{10.30} \\
        % \AlgoNameBLIP & \textbf{55.21} & \textbf{56.32} & \textbf{44.44} & \textbf{11.88} \\
        \bottomrule
    \end{tabular}
    }
\egroup
\vspace{-0.2cm}
\tiny
\vspace{-0.1cm}
\caption{Ablation studies on COCO Captions and TextCap}
\label{tab:caps_ablations}
\vspace{-0.7cm}
\end{center}
\end{table}

==> Rebuttal_Tables/rebuttal_subset.tex <==
\begin{table}
\normalsize
\begin{center}

\tiny
\bgroup
\def\arraystretch{1.1}
    \resizebox{0.8\linewidth}{!}{%
        \begin{tabular}{l | ccc}
        \toprule
        \textbf{Method} & \textbf{TextVQA} &
        \textbf{$\text{TextVQA}_{\text{Read}}$} & \textbf{$\text{TextVQA}_{\text{See}\boldsymbol{\cap}\text{Read}}$}\\ 
        \midrule
        % ALBEF \cite{albef} & 12.31 & 5.77 & \color{Red}{6.54} \\
        % BLIP \cite{li2022blip} & 21.12 & 15.19 & \color{Red}{5.93}\\
        % OFA \cite{ofa} & 17.07 & 13.27 & \color{Red}{3.80} \\
        M4C comb.  & 47.22 & 48.04 & 39.47 \\
        BLIP comb. & 32.43 & 33.13 & 25.87 \\
        \midrule
        % \AlgoNameALBEF & 44.07 & 33.77 & \textbf{10.30} \\
        \AlgoNameBLIP & \textbf{55.21} & \textbf{56.32} & \textbf{44.44} \\
        \bottomrule
    \end{tabular}
    }
\egroup
\vspace{-0.2cm}
\tiny
\caption{Subset evaluation on M4C and BLIP under the Comb. setting.}
\label{tab:rebuttal_subset}
\vspace{-0.9cm}
\end{center}
\end{table}

==> Rebuttal_Tables/unified_table.tex <==
\begin{table}[ht!]
\vspace{-0.2cm}
    \begin{subtable}[ht!]{0.5\linewidth}
        \centering
        \resizebox{1\linewidth}{!}{%
        \begin{tabular}{l | ccc}
                \firsthline
                \toprule
                % \textbf{Method} & \textbf{TextVQA} & \textbf{$\text{TextVQA}_{\text{Read}}$} & \textbf{$\text{TextVQA}_{\text{See}\boldsymbol{\cap}\text{Read}}$}\\ 
                \textbf{Method} & \textbf{See $\cup$ Read} & \textbf{Read} & \textbf{See $\cap$ Read}\\ 
                \midrule
                M4C comb.  & 47.22 & 48.04 & 39.47 \\
                BLIP comb. & 32.43 & 33.13 & 25.87 \\
                \midrule
                % \AlgoNameALBEF & 44.07 & 33.77 & \textbf{10.30} \\
                \AlgoNameBLIP & \textbf{55.21} & \textbf{56.32} & \textbf{44.44} \\
                \bottomrule
            \end{tabular}
        }
    \caption{Additional subset results}
    \label{tab:rebuttal_subset}
    \end{subtable}
%
    \hfill
    \begin{subtable}[ht]{0.45\linewidth}
    	\centering
    	\resizebox{1\linewidth}{!}{%
    	\begin{tabular}	{l | c c}
                \firsthline
                \toprule	 	
                \textbf{Method} &  \textbf{COCO} & \textbf{TextCaps} \\
                \midrule
                $\text{BLIP}_{\text{large}}$  & 136.7 & 60.04\\
                + Comb.  & 136.2 & 92.09 \\
                + \AlgoName  & \textbf{136.8} & \textbf{105.71} \\
        	\bottomrule
            \end{tabular}
            }
    \caption{UniTnT on BLIP-Large}
    \label{table:blip_large}
    \end{subtable}
\vspace{-0.2cm}
\end{table}

==> Rebuttal_Tables/unified_table2.tex <==
\begin{table}[!t]
\centering
\begin{subtable}{.5\linewidth}
\centering
% \captionsetup{width=.9\linewidth}
\begin{adjustbox}{max width=0.9\linewidth}
	    \begin{tabular}{l | ccc}
                \firsthline
                \toprule
                % \textbf{Method} & \textbf{TextVQA} & \textbf{$\text{TextVQA}_{\text{Read}}$} & \textbf{$\text{TextVQA}_{\text{See}\boldsymbol{\cap}\text{Read}}$}\\ 
                \textbf{Method} & \textbf{See $\cup$ Read} & \textbf{Read} & \textbf{See $\cap$ Read}\\ 
                \midrule
                M4C comb.  & 47.22 & 48.04 & 39.47 \\
                BLIP comb. & 32.43 & 33.13 & 25.87 \\
                \midrule
                % \AlgoNameALBEF & 44.07 & 33.77 & \textbf{10.30} \\
                \AlgoNameBLIP & \textbf{55.21} & \textbf{56.32} & \textbf{44.44} \\
                \bottomrule
            \end{tabular}
\end{adjustbox}
\vspace{-0.1cm}
\tiny
\caption{Additional subset results}
\label{tab:rebuttal_subset}
\end{subtable}
\begin{subtable}{.45\linewidth}
\centering
% \captionsetup{width=.9\linewidth}
\begin{adjustbox}{max width=0.9\linewidth}
	    \begin{tabular}	{l | c c}
                \firsthline
                \toprule	 	
                \textbf{Method} &  \textbf{COCO} & \textbf{TextCaps} \\
                \midrule
                $\text{BLIP}_{\text{large}}$  & 136.7 & 60.04\\
                + Comb.  & 136.2 & 92.09 \\
                + \AlgoName  & \textbf{136.8} & \textbf{105.71} \\
        	\bottomrule
            \end{tabular}
\end{adjustbox}
\vspace{-0.1cm}
\tiny
\caption{UniTnT on BLIP$_\text{Large}$}
\label{table:blip_large}
\end{subtable}
\vspace{-0.3cm}
\tiny
\caption{Additional requested experimental results}
\vspace{-0.7cm}
\end{table}

==> Tables/caps_textcaps_combined.tex <==


\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{@{\extracolsep{1pt}} l c | c c c| c }
        \toprule	 	
        \multirow{2}{*}{\textbf{Method}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} & \textbf{COCO} & \multicolumn{2}{c}{\textbf{TextCaps}} & \textbf{Avg.} \\ 
         & & Karpathy-test & val & test & \\
        \midrule
        M4C-Captioner~\cite{hu2020iterative}
        & \checkmark & 4.7 & 95.5 & 90.1 & 47.4  \\
        TAP~\cite{yang2021tap}
        & \checkmark & 4.6 & 109.2 & 103.2 & 53.9  \\
        OFA~\cite{ofa} & \ding{55} & 146.7 & 56.2 & 56.4 & 101.6  \\
        BLIP~\cite{li2022blip} & \ding{55} & 133.3 & 59.4 & 61.9 & 97.6  \\
	    \bottomrule
	\end{tabular}
	}
	\caption{\textbf{CAP models current status} The results of leading scene text and general models on scene text and general CAP benchmarks, revealing that currently, no method performs well on both.}
	\label{table:cap_textcap_combined}
\end{table}

==> Tables/component_ablations.tex <==
\begin{table}
\normalsize
\begin{center}

\small
\bgroup
\def\arraystretch{1.1}
    \resizebox{1\linewidth}{!}{%
        \begin{tabular}{cccccc | cc}
        \toprule
        \textbf{OCR-Sys} & \textbf{OCR-Enc} & \textbf{Fuse} & $\bm{\mathcal{L}_{OCR-LM}}$ & $\bm{\mathcal{L}_{OCR-BC}}$ & \textbf{2-D} &  \textbf{VQA} & \textbf{TextVQA} \\ 
        \midrule
        \ding{55} & \ding{55} & \ding{55} &\ding{55}  &\ding{55} & \ding{55} & 77.40 & 32.43 \\
        \checkmark & \ding{55} & \ding{55} &\ding{55}  &\ding{55} & \ding{55} & 77.66 & 43.02 \\
        \checkmark & \checkmark & \ding{55}  & \ding{55}  & \ding{55} & \ding{55} & 78.41 & 46.13 \\
        \checkmark & \checkmark & \checkmark  & \ding{55}  & \ding{55} & \ding{55} & 78.65 & 47.38 \\
        % \cdashline{2-8}
        \checkmark & \checkmark & \checkmark & \checkmark  & \ding{55} & \ding{55} & 79.86 & 52.66 \\
        \checkmark & \checkmark & \checkmark & \checkmark  & \checkmark & \ding{55} & 79.81 & 52.66 \\
        \checkmark & \checkmark & \checkmark & \checkmark  & \ding{55} & \checkmark & 79.74 & 52.93 \\
        \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 79.90  & 55.21 \\
        \bottomrule
    \end{tabular}
    }
\egroup
\vspace{-0.2cm}
\tiny
\caption{\textbf{\AlgoName design choices.} \AlgoNameBLIP accuracy on VQA and TextVQA (test-dev and validation) while sequentially adding the different building blocks of our method.}
\label{tab:main_blocks_ablation}
% \vspace{-0.7cm}
\end{center}
\end{table}

==> Tables/current_status.tex <==
\begin{table*}[!t]
\centering
\begin{subtable}{.5\textwidth}
\centering
\captionsetup{width=0.95\linewidth}
\begin{adjustbox}{max width=0.95\textwidth}
	\begin{tabular}	{l l c| c c c c c | c}
        \toprule	 	
        & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} &  \multicolumn{2}{c}{\textbf{VQA}} & \multicolumn{2}{c}{\textbf{TextVQA}} & \textbf{ST-VQA} & \multirow{2}{*}{\textbf{Avg.}} \\
        & & & test-dev & test-std & val & test & test-ANLS & \\
        \midrule
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Separate}}}}
        & M4C~\cite{hu2020iterative} & \checkmark & 27.47 & 27.70 & 46.53 & 47.42 & 0.43 & 37.56 \\
        & TAP~\cite{yang2021tap} & \checkmark & 18.76 & 18.81 & 54.71 & 53.97 & 0.60 & 36.39 \\
        & ALBEF~\cite{albef} & \ding{55} & 75.22 & 75.38 &  11.67 & 13.88 & 0.19 & 44.63 \\
        & BLIP~\cite{li2022blip} & \ding{55} & 76.39 & 76.59 &  20.50 & 23.74 & 0.34 & 50.16 \\
        & $\text{OFA}_{\text{Large}}$~\cite{ofa} & \ding{55} & 79.70 & 79.85 &  22.1 & 21.47 & 0.27 & 50.66 \\
        \hline
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Comb.}}}}
        & M4C \cite{hu2020iterative} & \checkmark & 59.11 & 59.04 & 47.22 & 48.61 & 0.50 & 53.83 \\
        & ALBEF \cite{albef} & \ding{55} & 75.61 & 75.87 & 16.15 & 17.04 & 0.22 & 46.46 \\
        & BLIP \cite{li2022blip} & \ding{55} & 77.40 & 77.39 &  32.43 & 31.48 & 0.44 & 54.44 \\
	    \bottomrule
	\end{tabular}
\end{adjustbox}
\caption{Accuracy/ANLS scores on VQA benchmarks. The average is taken over VQA test-std and TextVQA test accuracies.}
\label{table:vqa_textvqa_status}
\end{subtable}% <---- don't forget this %
\begin{subtable}{.5\textwidth}
\centering
\captionsetup{width=0.95\linewidth}
\begin{adjustbox}{max width=0.95\textwidth}
	\begin{tabular}	{l l c | c c c | c }
        \toprule	 	
        & \multirow{2}{*}{\textbf{Method}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} & \textbf{COCO} & \multicolumn{2}{c|}{\textbf{TextCaps}} & \multirow{2}{*}{\textbf{Avg.}} \\ 
        & & & Karpathy-test & val & test & \\
        \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Separate}}}}
        & M4C-Captioner~\cite{sidorov2020textcaps}
        & \checkmark & 4.7 & 95.5 & 90.1 & 47.4  \\
        & TAP~\cite{yang2021tap}
        & \checkmark & 4.6 & 109.2 & 103.2 & 53.9  \\
        & BLIP~\cite{li2022blip} & \ding{55} & 133.3 & 59.4 & 61.9 & 97.6  \\
        & $\text{OFA}_{\text{Large}}$~\cite{ofa} & \ding{55} & 150.7 & 64.5 & 66.8 & 108.8  \\
        \hline
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Comb.}}}}
        & M4C-Captioner \cite{sidorov2020textcaps} & \checkmark & 109.8 & 102.7 & 98.0 & 103.9  \\
        & BLIP \cite{li2022blip} & \ding{55} & 133.4 & 101.4 & 91.8 & 112.6 \\
	    \bottomrule
	\end{tabular}
\end{adjustbox}
\caption{CIDEr scores on image captioning benchmarks. The average is taken over COCO and TextCaps test scores.}

\label{table:cap_textcap_status}
\end{subtable}
\caption{\textbf{Current status of VQA and CAP models.} The results of leading methods
% \cite{hu2020iterative,sidorov2020textcaps,yang2021tap,albef,li2022blip,ofa}
on both scene-text and general VQA and CAP benchmarks, revealing that currently, no method performs well on both scene-text and general benchmarks.}
\label{tab:current_status}
\end{table*}

==> Tables/disentangling.tex <==
\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{@{\extracolsep{1pt}} l c c | c c | c}
        \toprule	 	
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{use} \\ \textbf{VQA}}} & \multirow{2}{*}{\shortstack[c]{\textbf{use} \\ \textbf{TextVQA}}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{VQA} \\ test-dev}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{TextVQA} \\ val}} & \multirow{2}{*}{\textbf{Avg.}} \\
        & & & & &  \\ 
        \midrule
        BLIP  & \multirow{2}{*}{\ding{55}} & \multirow{2}{*}{\checkmark}  & 36.53 & 32.75 & 34.64  \\
        \AlgoNameBLIP  & & & 36.80 & 49.55 & 43.17  \\
         \cdashline{1-6}
        BLIP & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\ding{55}} & 76.39 & 20.50 & 48.45 \\
        \AlgoNameBLIP & & & 79.67 & 36.33 & 58.00 \\
         \cdashline{1-6}
        BLIP & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & 77.40 & 32.43 & 54.92 \\
        \AlgoNameBLIP & & & 79.90 & 55.21 & 67.56 \\
        \bottomrule
	\end{tabular}
	}
	\caption{\textbf{The impact of training data.} We show the effect of each dataset configuration for training our models.}
	\label{table:ds_effects}
\end{table}

==> Tables/ds_effects.tex <==
\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{@{\extracolsep{1pt}} l c c | c c | c}
        \toprule	 	
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{use} \\ \textbf{VQA}}} & \multirow{2}{*}{\shortstack[c]{\textbf{use} \\ \textbf{TextVQA}}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{VQA} \\ test-dev}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{TextVQA} \\ val}} & \multirow{2}{*}{\textbf{Avg.}} \\
        & & & & &  \\ 
        \cdashline{1-6}
        \multirow{8}{*}{\textbf{\AlgoNameBLIP}}  & \ding{55} & \checkmark  & 37.01 & 50.19 & 43.60  \\
        & \checkmark & \ding{55} & 79.68 & 36.33 & 58.01 \\
        & \checkmark & \checkmark & \textbf{79.90} & \textbf{55.21} & \textbf{67.56} \\
        \cmidrule{2-6}
        & \multirow{2}{*}{\shortstack[c]{\textbf{use} \\ \textbf{COCO Caps}}} & \multirow{2}{*}{\shortstack[c]{\textbf{use} \\ \textbf{TextCaps}}} &
        \multirow{2}{*}{\shortstack[c]{\textbf{COCO Caps} \\ val}} & \multirow{2}{*}{\shortstack[c]{\textbf{TextCaps} \\ val}} &
        \multirow{2}{*}{\textbf{Avg.}} \\
        & & & & &  \\ 
        \cdashline{2-6}
        & \ding{55} & \checkmark  & 70.4 & \textbf{130.5} & 100.5  \\
        & \checkmark & \ding{55} & 133.7 & 59.6 & 96.7 \\
        & \checkmark & \checkmark & \textbf{134.0} & 119.1 & \textbf{126.6} \\
        \bottomrule
	\end{tabular}
	}
	\caption{\textbf{The impact of training data.} We show the effect of each dataset configuration for training our models.}
	\label{table:ds_effects}
\end{table}




==> Tables/fuse_ablation.tex <==
\begin{table}
\normalsize
\begin{center}
\small
\bgroup
\def\arraystretch{1.1}
    \resizebox{1\linewidth}{!}{%
        \begin{tabular}{ccccccc}
        \toprule
        \textbf{Model} & \textbf{Enc-Dec Sup} & \textbf{Joint-CA} &\textbf{Sepeate-CA} & \textbf{$\alpha_{gate}$} &  \textbf{VQA} & \textbf{TextVQA} \\ 
        \midrule
        \multirow{6}{*}{\AlgoNameBLIP} & \ding{55} & \checkmark  &\ding{55} & \ding{55} &  \\
        & \ding{55} & \ding{55}  & \checkmark & \ding{55} &  & \\
        & \ding{55} & \ding{55}  & \checkmark & \checkmark &  & \\
        \cdashline{2-7}
        & \checkmark & \checkmark  & \ding{55} & \ding{55} &  & \\
        & \checkmark & \ding{55}  & \checkmark & \ding{55} &  & \\
        & \checkmark & \ding{55}  & \checkmark & \checkmark &  & \\
        \bottomrule
    \end{tabular}
    }
\egroup
\vspace{-0.2cm}
\tiny
\caption{\textbf{The Effect of the Fuse Mechanism.} We ablate our visual-OCR fuse approach on VQA and TextVQA.}
\label{tab:ablation}
% \vspace{-0.7cm}
\end{center}
\end{table}

==> Tables/image_text_caps.tex <==
\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{@{\extracolsep{1pt}}l l c | c c c | c }
        \toprule	 	
        & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} & \textbf{COCO} &  \multicolumn{2}{c|}{\textbf{TextCaps}} & \textbf{Avg.} \\ 
         & & & Karpathy-test & val & test & \\
        \midrule
        \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Caps}}}}
        & VinVL \cite{zhang2021vinvl} & \ding{55} & 129.3 & - & - & - \\
        & $\text{LEMON}_{\text{base}}$ \cite{hu2022scaling} & \ding{55} & 133.3 & - & - & - \\
        & $\text{GIT}_{\text{large}}^{\text{Cap}}$~\cite{wang2022git} & \ding{55} & 138.5 & - & - & - \\
        & BLIP \cite{li2022blip} & \ding{55} & 133.3 & 59.4 & 61.9 & 97.6 \\
        & $\text{SimVLM}_{\text{large}}$~\cite{wang2021simvlm} & \ding{55} & \underline{142.6} & - & - & - \\
        & $\text{OFA}_{\text{Large}}$ \cite{ofa} & \ding{55} & \textbf{150.7} & 64.5 & 66.8 & 108.8 \\
        \midrule
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize TextCaps}}}} & $\text{GIT}_{\text{large}}^{\text{TextCap}}$~\cite{wang2022git} & \ding{55} & - & 106.3 & - & - \\
        & MMA-SR~\cite{wang2020multimodal} &\checkmark & - & 98.0 & 88.0 & - \\
        & CNMT~\cite{anonymous2020challenge} & \checkmark & - & - & 93.0 & - \\
        & M4C-Captioner \cite{sidorov2020textcaps} & \checkmark & 4.7 & 95.5 & 90.1 & 47.4  \\
        & TAP \cite{yang2021tap} & \checkmark & 4.6 & \underline{109.2} & \underline{103.2} & 53.9 \\
        \midrule
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Comb.}}}}
        & M4C-Captioner \cite{sidorov2020textcaps} & \checkmark & 109.8 & 102.7 & 98.0 & 103.9  \\
        & BLIP \cite{li2022blip} & \ding{55} & 133.4 & 101.4 & 91.8 & \underline{112.6} \\
        
        \midrule
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{\footnotesize Ours}}}} 
        & \AlgoNameBLIP & \checkmark & 134.0 & \textbf{119.1} & \textbf{109.4} & \textbf{121.7}  \\
        % & $\quad \Delta$ & & $\uparrow0.7$  & $\uparrow59.7$  & $\uparrow47.5$ & $\uparrow24.1$  \\
        & $\quad \Delta$ & & $\uparrow0.6$  & $\uparrow11.7$  & $\uparrow17.6$ & $\uparrow9.1$  \\
	    \bottomrule
	\end{tabular}
	}
	\caption{\textbf{Evaluation results on  CAP.} Leading methods' CIDEr scores on the COCO Karpathy test split and TextCaps. $\Delta$ indicates improvement over the base architecture with combined training. Our method improves the base architecture results and obtains the best average score across general and scene-text captioning benchmarks.}
	\label{table:textcap_cap}
\end{table}



==> Tables/main_sota_tab.tex <==
% \begin{table*}[t]
% \centering
% % split the table into two with and without Rosetta
% \begin{tabular}{ l l l l c c }
%     \hline
%     Method & OCR System & Pretraining & Extra Finetune & Val Acc. & Test Acc.\\
%     % \hline
%     % LoRRA~\cite{singh2019towards} & Rosetta-ml & \ding{55}  &\ding{55}  & 26.56 & 27.63 \\
%     % MM-GNN~\cite{gao2020multi} & Rosetta-ml & \ding{55}  &\ding{55}  & 31.44 & 31.10 \\
%     % M4C~\cite{hu2020iterative} & Rosetta-en & \ding{55}  &\ding{55}  & 39.40 & 39.01 \\
%     % SMA~\cite{gao2020structured} & Rosetta-en & \ding{55}  &\ding{55}  & 40.05 & 40.66 \\
%     % CRN~\cite{liu2020cascade} & Rosetta-en & \ding{55}  &\ding{55}  & 40.39 & 40.96 \\
%     % LaAP-Net~\cite{han2020finding} & Rosetta-en & \ding{55}  &\ding{55}  & 40.68 & 40.54 \\
%     % M4C$^\dagger$~\cite{hu2020iterative} & Rosetta-en & \ding{55}  &\ding{55}  & 39.55 & - \\
%     % TAP~\cite{yang2021tap} & Rosetta-en & TextVQA &\ding{55}  & \eat{\zyang{44.06}}44.06 & - \\
%     % % \rowcolor{LightGray}
%     % % \AlgoName~(Ours) (No visual) & Rosetta-en & \ding{55}  &\ding{55}  & \eat{\zyang{44.06}}44.12 & - \\
%     % % \AlgoName~(Ours) (No visual)& Rosetta-en & 70M Doc. & \eat{\zyang{48.08}}48.08 & - \\
%     % M4C~\cite{hu2020iterative} & Rosetta-en &
%     % \ding{55} & ST-VQA & 40.55 & 40.46 \\
%     % LaAP-Net~\cite{han2020finding} & Rosetta-en & \ding{55} & ST-VQA & 41.02 & 40.54 \\
%     % \rowcolor{LightGray} \AlgoName-Base  & Rosetta-en & \ding{55}  &\ding{55}  & 44.06  & - \\
%     % \rowcolor{LightGray} \AlgoName-Base  & Rosetta-en & 70M Doc. &\ding{55}  &  48.38 & - \\
  

%     \hline
%     SA-M4C~\cite{kant2020spatially} & Google-OCR & \ding{55} & ST-VQA & 45.4 & 44.6 \\
%     SMA~\cite{gao2020structured} & SBD-Trans OCR & \ding{55} & ST-VQA & - & 45.51 \\
%     M4C~\cite{hu2020iterative} & Microsoft-OCR & \ding{55}  &\ding{55}  & 44.50 & 44.75 \\
%     M4C~\cite{hu2020iterative} &  Microsoft-OCR & \ding{55}  & ST-VQA & \eat{\zyang{45.22}} 45.22 & - \\

    
%     TAP~\cite{yang2021tap} & Microsoft-OCR & TextVQA  &\ding{55}  & 49.91 & 49.71 \\
%     TAP~\cite{yang2021tap} & Microsoft-OCR & TextVQA, ST-VQA &\ding{55}  & 50.57 & 50.71 \\
%     TAP~\cite{yang2021tap} & Microsoft-OCR & \small{TextVQA, ST-VQA, TextCaps, OCR-CC} &\ding{55}  & 54.71 & 53.97 \\
%     % \AlgoName~(Ours)  & Scene Text Textract & \ding{55}  &\ding{55}  &  & - \\
    
%     M4C~\cite{hu2020iterative} &  \OCRNameNoSpace & \ding{55}  & \ding{55} & 47.84 & - \\
        
%     \rowcolor{LightGray} \AlgoNameSpace-Base  & \OCRNameNoSpace & \ding{55}  & \ding{55}  & 50.37 & - \\
%     \rowcolor{LightGray} \AlgoNameSpace-Base  & \OCRNameNoSpace & TextVQA  & \ding{55}  & 51.09 & - \\
%     \rowcolor{LightGray} \AlgoNameSpace-Base  & \OCRNameNoSpace & \small{70M Doc.}  &\ding{55}  & 57.77 & 57.88 \\
%     % \AlgoName-Base  & Scene Text Textract & \small{70M Doc., TextVQA} & 58.48 & - \\
%     \rowcolor{LightGray} \AlgoNameCombined-Base  & \OCRNameNoSpace & \small{70M Doc.} & ST-VQA & 59.53 & 59.55 \\
%     \rowcolor{LightGray} \AlgoNameSpace-Large  & \OCRNameNoSpace & \small{70M Doc.} &\ding{55}  & 59.76 & 59.24 \\
%     \rowcolor{LightGray} \AlgoNameCombined-Large  & \OCRNameNoSpace & \small{70M Doc.}& ST-VQA  & \textbf{61.05} & \textbf{61.60}\\
    

%     \hline
% \end{tabular}
% \caption{Results on the TextVQA dataset~\cite{singh2019towards}}
% \vspace{-0.0in}
% \label{table:textvqa}
% \end{table*}

\begin{table*}
\normalsize
\begin{center}
\footnotesize
\bgroup
\def\arraystretch{1.1}
        \begin{tabular}{llllccc}
        \toprule
        \textbf{Method} & \textbf{OCR System} & \textbf{Pre-Training Data} & \textbf{Extra Finetune} & \textbf{No. of Param.} & \textbf{Val Acc.} & \textbf{Test Acc.}\\
        \midrule
        % LoRRA~\cite{singh2019towards} & Rosetta-ml & \ding{55}  &\ding{55}  & 26.56 & 27.63 \\
        % MM-GNN~\cite{gao2020multi} & Rosetta-ml & \ding{55}  &\ding{55}  & 31.44 & 31.10 \\
        M4C~\cite{hu2020iterative} & Rosetta-en & \ding{55}  &\ding{55}   & 200M & 39.40 & 39.01 \\
        SMA~\cite{gao2020structured} & Rosetta-en & \ding{55}  &\ding{55}  & - & 40.05 & 40.66 \\
        CRN~\cite{liu2020cascade} & Rosetta-en & \ding{55}  &\ding{55} & -  & 40.39 & 40.96 \\
        LaAP-Net~\cite{han2020finding} & Rosetta-en & \ding{55}  &\ding{55} & - & 40.68 & 40.54 \\
        TAP~\cite{yang2021tap} & Rosetta-en & TextVQA &\ding{55} & 200M & \eat{\zyang{44.06}}44.06 & - \\
        % M4C~\cite{hu2020iterative} & Rosetta-en & \ding{55}  &\ding{55}  & 39.55 & - \\
        % \rowcolor{LightGray}
        % \AlgoName~(Ours) (No visual) & Rosetta-en & \ding{55}  &\ding{55}  & \eat{\zyang{44.06}}44.12 & - \\
        % \AlgoName~(Ours) (No visual)& Rosetta-en & 70M Doc. & \eat{\zyang{48.08}}48.08 & - \\
        \rowcolor{LightGray} \AlgoName-Small  & Rosetta-en & \ding{55}  &\ding{55} & 149M & 41.84  & - \\
        \rowcolor{LightGray} \AlgoName-Base  & Rosetta-en & \ding{55}  &\ding{55} & 311M & 44.06  & - \\
        \rowcolor{LightGray} \AlgoName-Base  & Rosetta-en & IDL &\ding{55} & 311M &  48.38 & - \\
        \midrule
        SA-M4C~\cite{kant2020spatially} & Google-OCR & \ding{55} & ST-VQA & 200M & 45.4 & 44.6 \\
        SMA~\cite{gao2020structured} & SBD-Trans OCR & \ding{55} & ST-VQA & - & - & 45.51 \\
        % M4C~\cite{hu2020iterative} & Microsoft-OCR & \ding{55}  &\ding{55}  & 44.50 & 44.75 \\
        M4C~\cite{hu2020iterative,yang2021tap} &  Microsoft-OCR & \ding{55}  & ST-VQA & 200M & \eat{\zyang{45.22}} 45.22 & - \\
        TAP~\cite{yang2021tap} & Microsoft-OCR & TextVQA  &\ding{55}  & 200M & 49.91 & 49.71 \\
        TAP~\cite{yang2021tap} & Microsoft-OCR & TextVQA, ST-VQA & ST-VQA & 200M & 50.57 & 50.71 \\
        LOGOS~\cite{lu2021localize} & Microsoft-OCR & \ding{55} & ST-VQA & - & 51.53 & 51.08 \\
        TAP~\cite{yang2021tap} & Microsoft-OCR & TextVQA, ST-VQA, TextCaps, OCR-CC & ST-VQA  & 200M & 54.71 & 53.97 \\
        % \AlgoName~(Ours)  & Scene Text Textract & \ding{55}  &\ding{55}  &  & - \\
        
        M4C~\cite{hu2020iterative} &  \OCRNameNoSpace & \ding{55}  & \ding{55} & 200M & 47.84 & - \\
            
        \rowcolor{LightGray} \AlgoNameNoSpace-Base  & \OCRNameNoSpace & \ding{55}  & \ding{55} & 311M & 52.29 & - \\
        % \rowcolor{LightGray} \AlgoNameCombinedNoSpace-Base  & \OCRNameNoSpace & TextVQA, ST-VQA, TextCaps, OCR-CC & \ding{55}& 54.22 & - \\

        % % \rowcolor{LightGray} \AlgoNameNoSpace-Base  & \OCRNameNoSpace & TextVQA  & \ding{55}  & 51.09 & - \\
        % \rowcolor{LightGray} \AlgoNameCombinedNoSpace-Base  & \OCRNameNoSpace & IDL,TextVQA, ST-VQA, TextCaps, OCR-CC & \ding{55} & 58.51 & - \\
        % \rowcolor{LightGray} \AlgoNameCombinedNoSpace-Base  & \OCRNameNoSpace & IDL,TextVQA, ST-VQA, TextCaps, OCR-CC & ST-VQA & 59.06 & - \\
        % \AlgoName-Base  & Scene Text Textract & \small{70M Doc., TextVQA} & 58.48 & - \\
        \rowcolor{LightGray} \AlgoNameNoSpace-Base  & \OCRNameNoSpace & IDL  & \ding{55} & 311M & 58.03 & 58.86 \\
        \rowcolor{LightGray} \AlgoNameCombinedNoSpace-Base  & \OCRNameNoSpace & IDL & ST-VQA & 311M & 59.53 & 59.55 \\

        \rowcolor{LightGray} \AlgoNameNoSpace-Large  & \OCRNameNoSpace & IDL & \ding{55}  & 856M & 59.76 & 59.24 \\
        \rowcolor{LightGray} \AlgoNameCombinedNoSpace-Large  & \OCRNameNoSpace & IDL & ST-VQA & 856M & \textbf{61.05} & \textbf{61.60} \\
        % 770M + 83M + 3M
        \bottomrule
    \end{tabular}
\egroup
\vspace{-0.2cm}
\tiny
\caption{\textbf{Results on the TextVQA dataset~\cite{singh2019towards}}. As commonly done, the top part of the table presents results in the constrained setting that only uses TextVQA
for training and Rosetta for OCR detection, while the bottom part is the unconstrained settings. \AlgoName advances the state-of-the-art performance, specifically by +6.43\% and +7.63\% on validation and test, respectively.}
\label{table:textvqa}
\vspace{-0.8cm}
\end{center}
\end{table*}

==> Tables/vqa_textvqa.tex <==
\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{@{\extracolsep{1pt}}l l c | c c c c c | c}
        \toprule	 	
        & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} &  \multicolumn{2}{c}{\textbf{VQA}} & \multicolumn{2}{c}{\textbf{TextVQA}} & \textbf{ST-VQA} & \textbf{Avg.} \\
        & & & test-dev & test-std & val & test & test-ANLS & \\
        \midrule
        \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{\small VQA}}}} 
        & $\text{SimVLM}_{\text{large}}$ \cite{wang2021simvlm} & \ding{55} & \color{gray}{79.32} & \color{gray}{79.56} & - & - & - & - \\
        & $\text{GIT}_{\text{large}}^{\text{VQA}}$~\cite{wang2022git} & \ding{55} & 75.51 & - & - & - & - & - \\
        & ALBEF \cite{albef} & \ding{55} & 75.22 & 75.38 & 11.67 & 13.88 & 0.19 & 44.63 \\
        & BLIP \cite{li2022blip} & \ding{55} & 76.39 & 76.59 & 20.50 & 23.74 & 0.34 & 50.17 \\
        & $\text{OFA}_{\text{Large}}$~\cite{ofa} & \ding{55} & 79.70 & \underline{79.85} & 22.10 & 21.47 & 0.27 & 50.66 \\
        & $\text{mPLUG}_{\text{ViT-B}}$~\cite{li2022mplug} & \ding{55} & \color{gray}{\underline{79.79}} & \color{gray}{79.81} & - & - & - & - \\
        \midrule
        \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{\small TextVQA}}}} & $\text{GIT}_{\text{large}}^{\text{TextVQA}}$~\cite{wang2022git} & \ding{55} & - & - & 37.47 & - & - & - \\
        & SA-M4C\cite{kant2020spatially} & \checkmark & - & - & \color{gray}{45.4} & \color{gray}{44.6} & \color{gray}{0.50} & - \\
        & LOGOS \cite{lu2021localize} & \checkmark & - & - & \color{gray}{51.53} & \color{gray}{51.08} & \color{gray}{0.58} & - \\
        & M4C \cite{hu2020iterative} & \checkmark & \color{gray}{27.47} & \color{gray}{27.70} & \color{gray}{46.53} & \color{gray}{47.42} & \color{gray}{0.43} & 37.56 \\
        & TAP \cite{yang2021tap} & \checkmark & \color{gray}{18.76} & \color{gray}{18.81} & \color{gray}{54.71} & \color{gray}{53.97} & \color{gray}{0.60} & 36.39 \\
        & LaTr \cite{biten2022latr} & \checkmark & - & - & \textbf{59.53} & \textbf{59.55} & \textbf{0.68} & - \\
        \midrule
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\small Comb.}}}}
        & M4C \cite{hu2020iterative} & \checkmark & \color{gray}{59.11} & \color{gray}{59.04} & \color{gray}{47.22} & \color{gray}{48.61} & \color{gray}{0.50} & 53.83 \\
        & ALBEF \cite{albef} & \ding{55} & 75.61 & 75.87 & 16.15 & 17.04 & 0.22 & 46.46 \\
        & BLIP \cite{li2022blip} & \ding{55} & 77.40 & 77.39 &  32.43 & 31.48 & 0.44 & 54.44 \\
        \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{\small Ours}}}} & $\text{\AlgoNameNoSpaceALBEF}$ & \checkmark & 77.60 & 77.80 & 43.73 & 44.13& 0.58 & \underline{60.97} \\
        % & $\quad \Delta$  & & $\uparrow2.38$ & $\uparrow2.42$ & $\uparrow32.06$ & $\uparrow30.25$ & $\uparrow0.39$ & $\uparrow16.34$ \\
        & $\quad \Delta$  & & $\uparrow1.99$ & $\uparrow1.93$ & $\uparrow27.58$ & $\uparrow27.09$ & $\uparrow0.36$ & $\uparrow14.51$ \\
        & \AlgoNameBLIP  & \checkmark & \textbf{79.90} & \textbf{80.08} & \underline{55.21} & \underline{55.35} & \underline{0.66} & \textbf{67.72} \\
        % & $\quad \Delta$  & &$\uparrow3.51$ & $\uparrow3.49$ & $\uparrow34.71$ & $\uparrow31.61$ & $\uparrow0.32$ & $\uparrow17.55$ \\
        & $\quad \Delta$  & &$\uparrow2.50$ & $\uparrow2.69$ & $\uparrow22.77$ & $\uparrow23.87$ & $\uparrow0.22$ & $\uparrow13.28$ \\
	    \bottomrule
	\end{tabular}
	}
	\caption{\textbf{Results on VQA, TextVQA and ST-VQA.}
	% Top to bottom: the accuracy of general VQA methods, scene-text oriented approaches, our reimplemented models trained on both types of datasets, and our models.
     Accuracies of general VQA and scene-text oriented approaches trained with separate finetuning, models trained with combined finetuning, and \AlgoName. 
    Approaches that during inference use an answer pre-defined vocabulary are marked in {\color{gray}gray}. $\Delta$ indicates improvement over the base architecture trained using combined finetuning. Our method not only significantly improves the performance on scene-text tasks but also substantially increases the results on the general VQA ($\uparrow3.49\%$).}
	\label{table:vqa_textvqa}
\end{table}

==> Tables/vqa_textvqa_combined.tex <==
% \begin{table}[!t]
% 	\centering
% 	\resizebox{1\linewidth}{!}{%
% 	\begin{tabular}	{@{\extracolsep{1pt}}l c c| c c c c c c c | c}
%         \toprule	 	
%         \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{Combined} \\ \textbf{Training}}} & \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} &  \multicolumn{2}{c}{\textbf{VQA}} & \multicolumn{2}{c}{\textbf{TextVQA}} & \textbf{ST-VQA} & \textbf{Avg.} \\
%         & & & test-dev & test-std & val & test & test-ANLS & \\
%         \midrule
%         \multirow{2}{*}{{M4C~\cite{hu2020iterative}}} & \ding{55} & \checkmark & 27.47 & 27.70 & 46.53 & 47.42 & 0.43 & 37.56 \\
%         & \checkmark & \checkmark & \textbf{59.11} & \textbf{59.04} & \textbf{47.22} & \textbf{48.61} & \textbf{0.50} & ? \\
%         \cdashline{1-9}
        
%         \multirow{2}{*}{{BLIP~\cite{li2022blip}}} & \ding{55} & \ding{55} & 76.39 & 76.59 &  20.50 & 23.74 & 0.34 & 50.16 \\
%         & \checkmark & \ding{55} & \textbf{77.40} & \textbf{77.39} &  \textbf{32.43} & \textbf{31.48} & \textbf{0.44} & \textbf{54.43} \\
%         % \cdashline{1-9}
        
%         % \multirow{2}{*}{{$\text{OFA}_{\text{Base}}$~\cite{ofa}}} & \ding{55} & \ding{55} & ? & ? & ? & ? & ? & ? \\
%         % & \checkmark & \ding{55} & ? & ? & ? & ? & ? & ? \\
% 	    \bottomrule
% 	\end{tabular}
% 	}
% 	\caption{\textbf{Results on ST non-ST VQA combined training.} Each method is finetuned twice -- once on ST (M4C) / non-ST (BLIP) and once on the unified dataset.}
% 	\label{table:vqa_textvqa_combined}
% \end{table}

\begin{table}[!t]
	\centering
	\resizebox{1\linewidth}{!}{%
	\begin{tabular}	{@{\extracolsep{1pt}}l c| c c c c c | c}
        \toprule	 	
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{OCR} \\ \textbf{System}}} &  \multicolumn{2}{c}{\textbf{VQA}} & \multicolumn{2}{c}{\textbf{TextVQA}} & \textbf{ST-VQA} & \textbf{Avg.} \\
        & & test-dev & test-std & val & test & test-ANLS & \\
        \midrule
        M4C~\cite{hu2020iterative} & \checkmark & 27.47 & 27.70 & 46.53 & 47.42 & 0.43 & 37.56 \\
        TAP~\cite{yang2021tap} & \checkmark & 18.76 & 18.81 & 54.71 & 53.97 & 0.60 & 36.39 \\
        ALBEF~\cite{albef} & \ding{55} & 75.22 & 75.38 &  11.67 & 13.88 & 0.19 & 44.63 \\
        OFA~\cite{ofa} & \ding{55} & 77.4 & 77.6 &  16.7 & 16.9 & 0.22 & 47.25 \\
        BLIP~\cite{li2022blip} & \ding{55} & 76.39 & 76.59 &  20.50 & 23.74 & 0.34 & 50.16 \\
        % \cdashline{1-9}
        
        % \multirow{2}{*}{{$\text{OFA}_{\text{Base}}$~\cite{ofa}}} & \ding{55} & \ding{55} & ? & ? & ? & ? & ? & ? \\
        % & \checkmark & \ding{55} & ? & ? & ? & ? & ? & ? \\
	    \bottomrule
	\end{tabular}
	}
% 	\caption{\textbf{Results on scene text and general VQA benchmarks.} We examine the performance of leading scene text and general VQA models on both benchmarks and reveal that no current method performs well on both.}
    \caption{\textbf{VQA models current status} The results of leading scene text and general models on scene text and general VQA benchmarks, revealing that currently, no method performs well on both.}
	\label{table:vqa_textvqa_combined}
\end{table}
